LazyDiT: Lazy Learning for the Acceleration of Diffusion Transformers

Diffusion Transformers have emerged as the preeminent models for a wide array of generative tasks, demonstrating superior performance and efficacy across various applications. The promising results come at the cost of slow inference, as each denoising step requires running the whole transformer model with a large amount of parameters. In this paper, we show that performing the full computation of the model at each diffusion step is unnecessary, as some computations can be skipped by lazily reusing the results of previous steps. Furthermore, we show that the lower bound of similarity between outputs at consecutive steps is notably high, and this similarity can be linearly approximated using the inputs. To verify our demonstrations, we propose the \textbf{LazyDiT}, a lazy learning framework that efficiently leverages cached results from earlier steps to skip redundant computations. Specifically, we incorporate lazy learning layers into the model, effectively trained to maximize laziness, enabling dynamic skipping of redundant computations. Experimental results show that LazyDiT outperforms the DDIM sampler across multiple diffusion transformer models at various resolutions. Furthermore, we implement our method on mobile devices, achieving better performance than DDIM with similar latency. Code: https://github.com/shawnricecake/lazydit

==> sections/10-rebuttal.tex <==




\section*{Reviewer K9CR (7)}

\subsection*{Rebuttal 1}
\subsubsection{Weakness}
The idea of lazy evaluation is not novel; similar caching or lazy evaluation techniques exist in other fields, which may limit the originality of the approach.

\subsubsection{Rebuttal}
Many thanks  for the constructive feedback. We highlight our novelty below. 
(i) \textbf{Application for Transformers.} While cache mechanisms have indeed been explored in UNet-based diffusion models, their application in transformer-based diffusion models remains underexplored. 
(ii) \textbf{Theoretic analysis.} Our work aims to bridge this gap by rigorously analyzing the mathematical similarities across diffusion steps specifically within the transformer architectures, which has not been the focus of prior research. Our theorems leverage the Lipschitz continuity of the MHSA and Feedforward layers to show that successive steps are similar. This similarity allows us to safely use the previous cache, thereby saving computation.  Previous works explore caching with experiments, lacking deep insights for the rational of caching. 
(iii) \textbf{Dynamic skip mechanisms.}  Our primary contribution is establishing a formal mathematical foundation for dynamic cache mechanisms in transformer-based diffusion, offering a theoretical basis for future optimizations and model efficiency improvements. Our mathematical analysis 
in Theorem 3 at Section 3.2
\textcolor{red}{(Line or Section XXXX)} 
reveals that diffusion step similarity is input-dependent and based on that, we design a dynamic skip strategy to use different skip strategies for different inputs, unlike prior arts such as DeepCache and Learn2Cache with the same skip for all inputs. 

\textbf{Summary.} We validate this theory with empirical methods, verifying the effectiveness of dynamic caching strategies with transformers, which we believe is a novel and impactful advancement.
Thank you again for the opportunity to clarify our contributions.



\section*{Reviewer pAJj (5)}

\subsection*{Rebuttal 1}
\subsubsection{Weakness}
Cache-based methods [1] [2], are widely recognized, yet this paper does not adequately discuss these methods in the introduction or related work sections. Additionally, the first claimed contribution seems to overlap with what has already been extensively addressed by prior research, which may reduce the perceived novelty of the work. A more thorough review of existing cache-based strategies would help to clarify the unique contributions of this research.

[1] Cache Me if You Can: Accelerating Diffusion Models through Block Caching 

[2] DeepCache: Accelerating Diffusion Models for Free 

[3] Learning-to-Cache: Accelerating Diffusion Transformer via Layer Caching

[4] All are Worth Words: A ViT Backbone for Diffusion Models

\subsubsection{Rebuttal}
Thanks for your question. We highlight that our method differs from previous works such as [1,2,3] in four ways:   (i) \textbf{Theoretic analysis.} We provide a theoretic analysis  to demonstrate the effectiveness of caching.
% , while previous works are experimental. 
Theorem 1 demonstrates that appropriate scaling and shifting parameters can bound the distance between two consecutive diffusion steps. 
Theorem 2 further leverages Lipschitz continuity of MHSA and Feedforward layers to show that successive steps are similar, which allows to use previous cache.
% This similarity allows us to safely use the previous cache, thereby saving computation.  
While previous works explore caching with experiments, lacking deep insights.
% for the rational of caching. 

(ii) \textbf{Applications for Transformers.} Our method focuses on transformer-based diffusion models with flexibility to extend to other architectures such as U-ViT [4].
While prior works [1,2] are designed for UNet-based.
% models rather than transformer-based ones. 

(iii) \textbf{Dynamic lazy skip.} Our lazy skip strategy are dynamic with 
% different skip strategies for 
different inputs, while other works such as [3] are static with the same skip strategy for all inputs.   
% Our mathematical analysis in 
The Theorem 3 reveals that diffusion step similarity is input-dependent.
% and based on that, we design a dynamic skip strategy corresponding to different inputs, unlike prior arts such as [3] with the same skip for different inputs. 

(iv) \textbf{Efficient training.} 
% Our method is more training efficient. 
Our method achieves efficient training using only a small subset of ImageNet samples with 500 steps on 8 GPUs within 10 minutes.
% completing training in 10 minutes on 8 GPUs.  
% By comparison, [3] needs to train on the full ImageNet with 1 epoch. 
By comparison, [3] needs full ImageNet and full epoch with 8 GPUs.
% The high training cost may limit the scalability of [3] for large models such as LargeDiT-3B or LargeDiT-7B.  However, Our efficient approach offers a scalable solution for these larger models.
High training costs limit the scalability of [3] for large models like LargeDiT-3B and LargeDiT-7B, whereas our method extends effectively to these models.

%Prior works, such as [1] and [2], have proposed methods specifically for UNet-based diffusion models rather than transformer-based ones. While [3] introduces a caching method for Diffusion Transformer (DiT), it is static with respect to inputs and relies on the whole ImageNet dataset for full training with 8 GPUs, limiting its general applicability beyond ImageNet.

%In our work, our mathematical analysis reveals that diffusion step similarity is input-dependent, not static, highlighting that [3] may overfit to ImageNet. 
%Our method achieves efficient training using only a small subset of ImageNet samples with 500 steps, completing training in 10 minutes on 8 GPUs.
%Meanwhile, the scalability of work [3] is restricted to models like LargeDiT-3B or LargeDiT-7B, which require more extensive model parameters and training data. Our approach, however, offers a scalable solution for these larger models.


\subsection*{Rebuttal 2}
\subsubsection{Weakness}
The work shares similarities with the "Learn2Cache" approach; however, key comparison results are relegated to the supplementary material rather than the main text. The experiments primarily compare the proposed method to older solvers, such as DDIM which is very limited. Incorporating a detailed analysis and comparison with "Learn2Cache" in the main results section would be essential for a more comprehensive evaluation of performance and effectiveness.

\subsubsection{Rebuttal}
Thanks for the suggestion. In the above discussion, we highlighted two key differences from Learn2Cache [3]: the use of a dynamic skip strategy and efficient training. 
% Here, we further compare the experimental results.

% (i) \textbf{Dynamic lazy skip.}
% Using Theorem 3, we employ a dynamic lazy skip strategy tailored to different inputs, whereas [3] uses a uniform skip strategy for all inputs.
% % Our lazy skip strategy are dynamic with different skip strategies for different inputs, while [3] is static with the same skip strategy for all inputs.   
% % Our mathematical analysis in Theorem 3 at Section 3.2 reveals that diffusion step similarity is input-dependent. Based on that, we design a dynamic skip strategy corresponding to different inputs, unlike  [3] with the same skip for different inputs. 
% (ii) \textbf{Efficient training.} 
% Unlike [3], which requires the entire ImageNet for training, our approach uses only a small subset, completing training in 10 minutes with just 500 steps, facilitating its extension to larger models
% % [3] requires entire ImageNet dataset for training, whereas our approach achieves effective results using only a small subset of ImageNet data, completing training in 10 minutes with only 500 steps. 
% % The expensive training of [3] may limit its application to larger models such as LargeDiT-3B and LargeDiT-7B with much more parameters.

% \textbf{Experimental comparison.}  We show our comparison with [3] in supplementary as it may not be fair enough due to their different training cost.  Additionally, we further compare with DPM-Solver-2 and Learn2Cache  for the U-ViT-H/2 model on ImageNet in 256×256 resolution.   As shown in the following Table, our method performs better than DPM-Solver-2 and Learn2Cache.  Although we use much less  training data than Learn2Cache, our superior  performance demonstrates the effectiveness of dynamic skipping   grounded on our theoretic analysis  than static skipping. Thanks for the suggestion, we will include a detailed comparison with Learn2Cache in the main paper in the revision.  

% For experiments compared to [3], we put them in supplementary as it may not be fair enough due to the different training cost. Additionally, we further compare with DPM-Solver-2 and [3] for the U-ViT-H/2 model on ImageNet in 256×256 resolution at following table. Although we use much less  training data than Learn2Cache, our superior performance demonstrates the effectiveness of dynamic skipping   grounded on our theoretic analysis  than static skipping. Thanks for the suggestion, we will include a detailed comparison with Learn2Cache in revision.

We include comparisons with [3] in the supplementary materials, as differences in training costs may affect fairness. We compare with DPM-Solver-2 and [3] for the U-ViT-H/2 model on 256×256 resolution in table below. Despite using significantly less training data than [3], our superior performance underscores the effectiveness of our theory-backed dynamic skipping over static skipping. Thank you for the suggestion, we will provide a detailed comparison with [3] in revision.


%As discussed, the "Learn2Cache" approach [3] is static rather than input-dependent, unlike our proposed method grounded in mathematical analysis. Additionally, "Learn2Cache" requires the entire ImageNet dataset for training, whereas our approach achieves effective results using only a small subset of ImageNet data, completing training in 10 minutes with only 500 steps. The difference in training cost is why we included our comparison in the supplementary material.

%Moreover, since "Learn2Cache" depends on the full training dataset, it faces scalability limitations and is unlikely to extend effectively to larger models, such as LargeDiT-3B and LargeDiT-7B, which contains significantly much more parameters for full training.


%Additionally, we provide the comparison with DPM-Solver-2 and Learn2Cache method with U-ViT-H/2 on ImageNet in 256×256 resolution as the following Table. The results show that our method performs better than DPM-Solver-2 and Learn2Cache.

% \textcolor{red}{todo: run experiment with U-ViT-H/2}
\begin{table}[]
\begin{tabular}{c|ccc|ccc}
Method      & NFE & MACs & FID $\downarrow$ & NFE & MACs & FID $\downarrow$  \\
\midrule
DPM-Solver  & 50  & 6.44 & 2.37 & 20  & 2.58 & 2.57 \\
DPM-Solver  & 30  & 3.86 & 2.46 & 16  & 2.06 & 2.7  \\
Learn2Cache & 50  & 3.79 & 2.36 & 20  & 1.92 & 2.58 \\
\midrule
Ours        & 50  & 3.87 & 2.35 & 20  & 2.06 & 2.52 \\
\end{tabular}
\end{table}




\subsection*{Rebuttal 3}
\subsubsection{Weakness}
There is insufficient detail regarding the efficiency and cost of the proposed method during the inference stage, especially when considering the associated training expenses. A comparison with other post-training cache-based methods is necessary to contextualize the trade-offs in terms of computation and resource utilization. Further elaboration on how the proposed strategy performs relative to these alternatives would strengthen the paper's argument for its efficiency and practicality
\subsubsection{Rebuttal}

% For the training cost, as  discussed in Section 4.1, we adopt a small subset of ImageNet with 500 training steps, which can be finished within 10 minutes with 8 GPUs. 
% %The details can be found in Section 4.1.
% On the other hand, Learn2Cache [3] method requires the whole ImageNet with a much more expensive training overhead, which may limit the extension to models with much more parameters such as LargeDiT-3B and LargeDiT-7B.

% As discussed in Section 4.1, we use a small subset of ImageNet with 500 training steps, completed in 10 minutes on 8 GPUs. In contrast, [3] requires the entire ImageNet and incurs higher training costs, limiting scalability to larger models like LargeDiT-3B and LargeDiT-7B.



% As for the inference cost, the latency results are shown in Table 3, and the comparison to Learn2Cache [3] method is included in Table 7 and Appendix A.3. Our results achieve better performance than Learn2Cache  in most cases. Especially, our method performs much bet-
% ter with less computation cost and higher inference speed when the resolution becomes 512×512.

%When the resolution becomes larger and the number of steps becomes lower, our method outperforms Learn2Cache method with less computation cost and higher inference speed, which shows the effectiveness of our method.

We discussed the training cost in above disscusion.
As for inference cost, the latency results are presented in Table 3. Comparison to [3] is included in Table 7 at Appendix A.3. Our method outperforms [3] in most cases, particularly at 512×512 resolution, where it achieves significantly better performance with lower computation cost and higher inference speed.


[1] Cache Me if You Can: Accelerating Diffusion Models through Block Caching 

[2] DeepCache: Accelerating Diffusion Models for Free 

[3] Learning-to-Cache: Accelerating Diffusion Transformer via Layer Caching

[4] All are Worth Words: A ViT Backbone for Diffusion Models




\section*{Reviewer 589R (7)}

\subsection*{Rebuttal 1}
\subsubsection{Recommendation}
This is a simple idea applied on diffusion Networks that seems to provide reasonable gains. The paper is well written, but some of the preliminary details such as DDIM and LDM have been rushed through, understandably due to lack of space. Perhaps this should be explained in further detail at least in the appendix.
\subsubsection{Answer}
Thanks for the suggestion, we will show the preliminary details of DDIM and LDM in supplementary in the revision.

\subsection*{Rebuttal 2}
\subsubsection{Question}
You have chosen to apply lazy layers for each of the Feed forward and attention layers in the main competition; why not apply a single lazy layer to approximate the entire network? If two successive iterations are indeed very similar then maybe a single layer can approximate the difference between those two iterations?

\subsubsection{Answer}
Many thanks for the question. We provide a visualization of the laziness in DiT models in Figure 4. This visualization reveals that, in  early layers, the MHSA module contributes less significantly than the Feedforward module, whereas in deeper layers, the Feedforward module becomes less important than MHSA. This variation in importance across layers makes it challenging to apply lazy layers consistently throughout the network, as the representational roles of MHSA and Feedforward differ substantially within a single step.


\subsection*{Rebuttal 3}
\subsubsection{Question}
You should provide some simple intuition to explain the idea behind theorems 1 and 2; it seems like the main point is just that these layers are continuous with bounded derivatives and so the difference between two successive iterations is small.

\subsubsection{Answer}
% \textcolor{red}{@yufa, please answer this question}

Thank you for your insightful observation. Your explanation is correct.
Theorem 1 demonstrates that appropriate scaling and shifting parameters can bound the distance between two consecutive diffusion steps. Building on this, Theorem 2 leverages the Lipschitz continuity of the MHSA and Feedforward layers to show that successive steps are similar. The Lipschitz property in Eq.~(4) represents the supremum of the first derivative, ensuring that changes between iterations are bounded.  This similarity allows us to safely use the previous cache, thereby saving computation.

\section*{Reviewer KV4c (6)}

\subsection*{Rebuttal 1}
\subsubsection{Weakness}
The idea of feature redundancy between steps in diffusion transformers is not novel. Prior work, such as [1], was released more than six months ago and had the same observation and main idea. And several other papers [2,3,4] have explored this redundancy before the submission of this paper. I think presenting this as the main contribution is not entirely rigorous (I recognize the novelty of the method). At the very least, comparisons with [1] are necessary.

\subsubsection{Rebuttal}

\textbf{Detailed comparison.} Thanks for the comment. We highlight that our method differs from previous works such as [1,2,3,4] in three ways:   
% (i) We provide a theoretic analysis  to demonstrate the effectiveness of caching, while previous works are experimental. Our Theorem 1 demonstrates that appropriate scaling and shifting parameters can bound the distance between two consecutive diffusion steps. Building on this, Theorem 2 leverages the Lipschitz continuity of the MHSA and Feedforward layers to show that successive steps are similar. This similarity allows us to safely use the previous cache, thereby saving computation.  Previous works explore caching with experiments, lacking deep insights for the adoption of caching. 
(i) We provide a theoretic analysis of caching while previous works are experimental. Theorem 1 demonstrates that appropriate scaling and shifting parameters can bound the distance between two consecutive diffusion steps. Theorem 2 leverages the Lipschitz continuity of the MHSA and Feedforward layers to show that successive steps are similar, enabling safe use of cached data to reduce computation.


% (ii) Our lazy skip strategy are dynamic with different skip strategies for different inputs, while most other methods such as [2,XXX] are static with the same skip strategy for all inputs. Our mathematical analysis (Line or Section XXXX) reveals that diffusion step similarity is input-dependent and based on that, we design a dynamic skip strategy corresponding to different inputs, unlike prior arts such as [2] with the same skip for different inputs. \textcolor{red}{(check and add more baselines from [1,2,3,4])}
(ii) Our lazy skip strategy is dynamic and adapts to different inputs, unlike static methods such as [2] that use the same strategy for all inputs. Theorem 3 shows that similarity is input-dependent, motivating the design of a dynamic skip strategy.


% (iii) Our method is more efficient. Our method achieves efficient training using only a small subset of ImageNet samples with 500 steps, completing training in 10 minutes on 8 GPUs.  By comparison, [2] needs to train on the full ImageNet with 1 epoch. The high training cost may limit  the scalability of [2] for large models such as LargeDiT-3B or LargeDiT-7B.  However, Our efficient approach offers a scalable solution for these larger models.   \textcolor{red}{(check and add more baselines from [1,2,3,4])}
(iii) We enables efficient training using a small subset of ImageNet with 500 steps finished in just 10 minutes on 8 GPUs. In contrast, [2] requires training on the full ImageNet for 1 epoch. This high costs hinder the scalability of [2] for larger models like LargeDiT-3B or LargeDiT-7B. In comparison, our approach achieves the results shown in Table 2.


\textbf{Summary.} 
% In this paper, we make a key contribution by developing a formal mathematical framework for dynamic caching mechanisms in transformer-based diffusion models. This foundation provides a rigorous basis for future advancements, enabling optimized performance and enhanced efficiency across model architectures. We validate this theory with comprehensive experiments, verifying the effectiveness of dynamic caching strategies with transformers.
In this paper, we contribute a formal mathematical framework for dynamic caching in transformer-based diffusion models, validated through comprehensive experiments.



\textbf{Experimental comparison.} 
% For the comparison, we include the work [2] into comparison in Table 7 in Appendix A.3, and our method achieves better performance than [2], especially when the resolution becomes large and number of steps becomes less. Here we also provide the comparison to the work [1] in the following table. We adopt 30 steps with 40\% lazy ratio, which results in similar computation reduction as the work [1]. 10k samples are generated for a fair comparison with [1]. The results show that our method achieves better performance than the work~[1] .

% \textcolor{red}{(list MACs in table?)} % add speed-up instead

For comparison, we include [2] in Table 7 in Appendix A.3. We achieve better performance, particularly at higher resolutions and with fewer steps. Below, we also compare with [1], using 30 steps and a 40\% lazy ratio for the similar speed-up. Our method achieves better performance.


% \textcolor{red}{todo: run exp with 10k samples eval, 30 steps with 40\% lazy ratio}
\begin{table}[]
\begin{tabular}{c|ccc}
Method & NFE & Speed-up & FID $\downarrow$   \\
\midrule
DDIM   & 30  & 1.0$\times$ & 14.76 \\
DDIM   & 20  & 1.5$\times$ & 17.69 \\
FRDiff & 30  & 1.6$\times$ & 16.71 \\
\midrule
Ours   & 30  & 1.6$\times$ & 16.37
\end{tabular}
\end{table}





\subsection*{Rebuttal 2}
\subsubsection{Weakness}
The experiments are limited to a single architecture (DiT, with large-DiT being similar to DiT), a single sampler (DDIM), and one dataset (ImageNet). More experiments, including different architectures (e.g., SD3, PixArt), different settings (such as text-to-image generation), and different samplers, are preferred.

[1] FRDiff : Feature Reuse for Universal Training-free Acceleration of Diffusion Models. 

[2] Learning-to-Cache: Accelerating Diffusion Transformer via Layer Caching. 

[3] $\Delta$-DiT: A Training-Free Acceleration Method Tailored for Diffusion Transformers. 

[4] FORA: Fast-Forward Caching in Diffusion Transformer Acceleration. 


\subsubsection{Rebuttal}
% Thanks for the suggestion. 
% Our approach focuses on transformer-based diffusion models with flexibility to extend to other architectures, such as U-ViT [1]. 
% We further  compare our proposed method  with Learn2Cache [2] and another sampler DPM-Solver-2 on another model U-ViT-H/2  in the following table. We do not experiment with Stable Diffusion 3, since the access to its training data is limited  and lower-quality data has a significant influence on the performance. 
% The results in the table show that our method is effective on U-ViT model and performs better than other methods.

Thank you for the suggestion. Our approach focuses on transformer-based diffusion models with flexibility to extend to other architectures like U-ViT [5]. We compare with [2] and another sampler DPM-Solver-2 using another model U-ViT-H/2 in table below. We achieve better performance. While, Stable Diffusion 3 remains DiT architecture.


%Regarding larger models like Stable Diffusion 3, access to training data for these models is limited. Since lower-quality data could impact our method's performance, we opted to validate our approach using the U-ViT model to demonstrate its potential for broader application.
%We further provide the results of our proposed method on U-ViT-H/2 with comparison to Learn2Cache [2] and DPM-Solver-2 in the following table. The results show that our method is effective on U-ViT model and performs better than other methods.

% \textcolor{red}{todo: copy the exp results of U-ViT in rebuttal 2}
\begin{table}[]
\begin{tabular}{c|ccc|ccc}
Method      & NFE & MACs & FID $\downarrow$ & NFE & MACs & FID $\downarrow$  \\
\midrule
DPM-Solver  & 50  & 6.44 & 2.37 & 20  & 2.58 & 2.57 \\
DPM-Solver  & 30  & 3.86 & 2.46 & 16  & 2.06 & 2.7  \\
Learn2Cache & 50  & 3.79 & 2.36 & 20  & 1.92 & 2.58 \\
\midrule
Ours        & 50  & 3.87 & 2.35 & 20  & 2.06 & 2.52
\end{tabular}
\end{table}

% \textcolor{red}{todo: say we can not get data of those high-level models (sd3) with same architecture, thus we did not provide results}

[5] All are Worth Words: A ViT Backbone for Diffusion Models

% [2] Learning-to-Cache: Accelerating Diffusion Transformer via Layer Caching.



==> sections/6-checklist.tex <==

% https://aaai.org/conference/aaai/aaai-25/aaai-25-reproducibility-checklist/

\clearpage

\section*{Reproducibility Checklist}



\subsection*{This paper}


\begin{itemize}
    
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (\textcolor{blue}{yes}/partial/no/NA)

    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (\textcolor{blue}{yes}/no)

    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (\textcolor{blue}{yes}/no)
    
\end{itemize}



\subsection*{Does this paper make theoretical contributions? (\textcolor{blue}{yes}/no)}

If yes, please complete the list below.

\begin{itemize}

    \item All assumptions and restrictions are stated clearly and formally. (\textcolor{blue}{yes}/partial/no)

    \item All novel claims are stated formally (e.g., in theorem statements). (\textcolor{blue}{yes}/partial/no)
    
    \item Proofs of all novel claims are included. (\textcolor{blue}{yes}/partial/no)
    
    \item Proof sketches or intuitions are given for complex and/or novel results. (\textcolor{blue}{yes}/partial/no)
    
    \item Appropriate citations to theoretical tools used are given. (\textcolor{blue}{yes}/partial/no)
    
    \item All theoretical claims are demonstrated empirically to hold. (\textcolor{blue}{yes}/partial/no/NA)
    
    \item All experimental code used to eliminate or disprove claims is included. (\textcolor{blue}{yes}/no/NA)

\end{itemize}




\subsection*{Does this paper rely on one or more datasets? (\textcolor{blue}{yes}/no)}

If yes, please complete the list below.

\begin{itemize}

    \item A motivation is given for why the experiments are conducted on the selected datasets (\textcolor{blue}{yes}/partial/no/NA)
    
    \item All novel datasets introduced in this paper are included in a data appendix. (yes/\textcolor{blue}{partial}/no/NA)
    
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (\textcolor{blue}{yes}/partial/no/NA)
    
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (\textcolor{blue}{yes}/no/NA)
    
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (\textcolor{blue}{yes}/partial/no/NA)
    
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/\textcolor{blue}{NA})

\end{itemize}


\subsection*{Does this paper include computational experiments? (\textcolor{blue}{yes}/no)}

If yes, please complete the list below.

\begin{itemize}

    \item Any code required for pre-processing data is included in the appendix. (yes/partial/\textcolor{blue}{no}).
    
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/\textcolor{blue}{partial}/no)
    
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (\textcolor{blue}{yes}/partial/no)
    
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (\textcolor{blue}{yes}/partial/no)
    
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (\textcolor{blue}{yes}/partial/no/NA)
    
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (\textcolor{blue}{yes}/partial/no)
    
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (\textcolor{blue}{yes}/partial/no)
    
    \item This paper states the number of algorithm runs used to compute each reported result. (\textcolor{blue}{yes}/no)
    
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/\textcolor{blue}{no})
    
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/\textcolor{blue}{partial}/no)
    
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (\textcolor{blue}{yes}/partial/no/NA)
    
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (\textcolor{blue}{yes}/partial/no/NA)

\end{itemize}












==> sections/trash.tex <==
\newpage
% \onecolumn %%%% make algorithm one column to help writing


\begin{algorithm}[!ht]
\caption{Jump algorithm at inference time}
\label{alg:jump_inference}
\begin{algorithmic}[1]
    \Procedure{Jump}{$X(T) \in \mathbb{R}^{B \times N \times D}, L, T \in \mathbb{N}_+$}
    \State \Comment{$B$ denotes the number of batches}
    \State \Comment{$N$ denotes the number of patches}
    \State \Comment{$D$ denotes the hidden dimension}
    \State \Comment{$T$ denotes the number of diffusion steps}
    \State \Comment{$L$ denotes the number of model layers in Transformer}
    % \State \Comment{$\Attn_i$ denotes attention module at $i$-th layer}
    % \State \Comment{$\MLP_i$ denotes MLP module at $i$-th layer}
    % \State \Comment{$\Jump_i^{\Attn}, \Jump_i^{\MLP}$ denotes the layer that estimate the score of jumping for attention/MLP module at $i$-th layer; it's a linear layer with output dimension $1$ and a sigmoid activation}
    \State \Comment{$\mathsf{F}_i$ denotes attention/MLP module at $i$-th layer; $\mathsf{F}_i(\cdot): \R^{B\times N\times D}\to \R^{B\times N\times D}$}
    \State \Comment{$\Jump_i$ denotes the layer that estimate the jumping probability for attention/MLP module at $i$-th layer;
    it's a linear layer with output dimension $1$ and a sigmoid activation, and then summed over the patch dimenstion;
    $\Jump_i(\cdot): \R^{B \times N \times D} \to [0,1]^{B}$}
    % \State \Comment{$\Jump_i^{\MLP}$ denotes the probability layer of jumping for MLP lalyer at $i$-th layer} 
    % \State \Comment{$\Jump(\cdot): \R^{B \times N \times D} \to [0,1]^{B}$}
    % \Yufa{probability layer, $\Jump(\cdot): \R^{B \times N \times D} \to [0,1]^{B \times N}$, it's a linear layer with output dimension $1$ and then a sigmoid activation.} 
    % \Zhao{This sentence in English is wrong.}
    \State \Comment{$S$ denotes DDIM scheduler}

    % \State {\color{blue} /* We must go through one diffusion step to store the cache. */}
    
    % \State $X(T)_{0} \gets X(T)$  \Comment{Input at diffusion step $T$}
    % \For{$i = 1 \to L$}
    %     \State $A(T)_{i} \gets X(T)_{i-1} + \Attn_i(X(T)_{i-1})$    \Comment{Residual connection around attention}
    %     \State $X(T)_{i} \gets A(T)_{i} + \MLP_i(A(T)_{i})$    \Comment{Residual connection around MLP}
    % \EndFor
    % \State $X(T-1) \gets S(X(T)_L, X(T),T)$ 

    \State {\color{blue} /* Jump algorithm at inference time. */}
    
    \For{$t = T \to 1$} \Comment{Interate diffusion steps}
        \State $X(t)_{0} \gets X(t)$ 
        \Comment{$X(t)$ means the input tensor at $t$ diffusion step}
        \For{$i = 1 \to L$} \Comment{Iterate model layers}
            %%%% attention
            % \Yufa{I will write this in mask way later.}
            % \State $p_i^\Attn \gets \sum_{j \in [N]} (\Jump_i^{\Attn}(X(t)_{i-1}))_{*,j}$
             
            % \Yufa{Sum $N$ dimension first. $p_i \in \R^B$ then create mask}
            % \State $p_i^\Attn \gets \Jump_i^{\Attn}(X(t)_{i-1})$ \Comment{$p_i^\Attn \in [0,1]^B$}
            % \If{$p_i^\Attn < 0.5$ and $\Cache_i^\Attn \neq \emptyset$}   
            % % \Comment{$p_i^{\Attn}(X(t)_{i-1}) \in [0,1]$}
            %     \State $A(t)_{i} \gets X(t)_{i-1} + \Cache_i^\Attn$ 
            %     \Comment{$A(t)_{i} \in \R^{B \times N \times D}$}
            % \Else
            %     \State $\Cache_i^\Attn \gets \Attn_i(X(t)_{i-1})$
            %     \State $A(t)_{i} \gets X(t)_{i-1} + \Cache_i^\Attn$ 
            % \EndIf
            
            %%%% MLP
            % \State $p_i^\MLP \gets \Jump_i^{\MLP}(A(t)_{i})$ \Comment{$p_i^\MLP \in [0,1]^B$}
            % \If{$p_i^\MLP < 0.5$ and $\Cache_i^\MLP \neq \emptyset$}
            %     \State $X(t)_{i} \gets A(t)_{i} + \Cache_i^\MLP$ 
            %     \Comment{$X(t)_{i} \in \R^{B \times N \times D}$}
            % \Else
            %     \State $\Cache_i^\MLP \gets \MLP_i(X(t)_{i-1})$ 
            %     \State $X(t)_{i} \gets A(t)_{i} + \Cache_i^\MLP$ 
            %     % \Yufa{Store the cache for $\MLP_i(A(t)_{i})$}
            % \EndIf

            %%% general case
            \State $p_i \gets \Jump_i(X(t)_{i-1})$ \Comment{$p_i \in [0,1]^B$}
            \For{$j = 1 \to B$}  \Comment{Iterate batchs} 
              \If{$(p_i)_j < 0.5$ and $ (\Cache_i)_j \neq \emptyset$}
                \State \Comment{Reuse the cache of previous diffusion step to reduce computation if the jumping probability is less than $0.5$} 
                \State $(X(t)_{i})_{j} \gets (X(t)_{i-1})_{j} + (\Cache_i)_{j}$ 
                \Comment{$X(t)_{i} \in \R^{B \times N \times D}$ is the tensor at $i$-th layer; $(X(t)_{i})_j \in \R^{N \times D}$ is $j$-th batch of $X(t)_{i}$}
            \Else
                \State \Comment{Pass the attention/MLP layer if the jumping probability is greater than $0.5$}
                \State $(\Cache_i)_j \gets \mathsf{F}_i((X(t)_{i-1})_j)$ \Comment{Pass attention/MLP layer and store the cache}
                \State $(X(t)_{i})_j \gets (X(t)_{i-1})_j + (\Cache_i)_j$ \Comment{Residual connection}
            \EndIf

            
            % \If{$p_i < 0.5$ and $\Cache_i \neq \emptyset$}
            %     \State \Comment{Reuse the cache of previous diffusion step to reduce computation if the jumping probability is less than $0.5$} 
            %     \State $X(t)_{i} \gets X(t)_{i-1} + \Cache_i$ 
            %     \Comment{$X(t)_{i} \in \R^{B \times N \times D}$}
            % \Else
            %     \State \Comment{Pass the attention/MLP layer if the jumping probability is greater than $0.5$}
            %     \State $\Cache_i \gets \mathsf{F}_i(X(t)_{i-1})$ \Comment{Pass attention/MLP layer and store the cache}
            %     \State $X(t)_{i} \gets X(t)_{i-1} + \Cache_i$ \Comment{Residual connection}
            % \EndIf
        \EndFor    
        \EndFor
        \State $X(t-1) \gets S(X(t)_L, X(t),t)$ \Comment{Predict and remove noise} 
    \EndFor

    \State \Return $X(0)$ \Comment{The generated image}
    \EndProcedure
\end{algorithmic}
\end{algorithm}

% \Yufa{I will add another algorithm for training algorithm.}

% \Yufa{
% % \begin{align*}
% %     \mathrm{Loss} = \mathrm{DiffusionLoss} +  \rho^\Attn \sum_{i \in [B]} \mathrm{Mask}^\Attn_i +  \rho^\MLP \sum_{i \in [B]} \mathrm{Mask}^\MLP_i
% % \end{align*}

% \begin{align*}
%     \mathrm{Loss} = \mathrm{DiffusionLoss} +  \rho \sum_{i \in [B]} \|p_i\|_2
% \end{align*}
% % $\rho^\Attn = 1e-3$
% $\rho = 1e-3$
% % $\rho^\MLP = 1e-3$
% $p_i \in \R^B$
% }

\begin{algorithm}[!ht]
\caption{Jump algorithm at training time}
\label{alg:jump_train}
\begin{algorithmic}[1]
    \Procedure{Jump}{$X(T) \in \mathbb{R}^{B \times N \times D}, L, T \in \mathbb{N}_+$}
    \State \Comment{$B$ denotes the number of batches}
    \State \Comment{$N$ denotes the number of patches}
    \State \Comment{$D$ denotes the hidden dimension}
    \State \Comment{$T$ denotes the number of diffusion steps}
    \State \Comment{$L$ denotes the number of model layers in Transformer}
    \State \Comment{$\mathsf{F}_i$ denotes attention/MLP module at $i$-th layer; $\mathsf{F}_i(\cdot): \R^{B\times N\times D}\to \R^{B\times N\times D}$}
    \State \Comment{$\Jump_i$ denotes the layer that estimate the jumping probability for attention/MLP module at $i$-th layer;
    $\Jump_i(\cdot): \R^{B \times N \times D} \to [0,1]^{B}$}
    \State \Comment{$S$ denotes DDIM scheduler}
    \State {\color{blue} /* Jump algorithm at training time. */}

    % \For{$i = 1 \to L$} 
    %     \State  $\Cache_i \gets 0^{B\times N\times D}$
    % \EndFor
    
    \For{$t = T \to 1$} \Comment{Iterate diffusion steps}
        \State $X(t)_{0} \gets X(t)$ 
        \For{$i = 1 \to L$} \Comment{Iterate model layers}
            \State $p_i \gets \Jump_i(X(t)_{i-1})$ \Comment{$p_i \in [0,1]^B$}
            \For{$j = 1 \to B$}  \Comment{Iterate batchs} 
            
            \If{$ (\Cache_i)_j = \emptyset$}
                \State $(\Cache_i)_j \gets \mathsf{F}_i((X(t)_{i-1})_j)$
                \State $(X(t)_{i})_j \gets (X(t)_{i-1})_j +  (\Cache_i)_j$
            \Else
                \State $(X(t)_{i})_j \gets (X(t)_{i-1})_j +(1 - (p_i)_j) \cdot (\Cache_i)_j + (p_i)_j \cdot \mathsf{F}_i((X(t)_{i-1})_j)$
                \State $(\Cache_i)_j \gets \mathsf{F}_i((X(t)_{i-1})_j)$ 
            \EndIf
            
        \EndFor    
        \EndFor
        \State $X(t-1) \gets S(X(t)_L, X(t),t)$ \Comment{Predict and remove noise} 
    \EndFor

    \State \Return $X(0)$ \Comment{The generated image}
    \EndProcedure
\end{algorithmic}
\end{algorithm}



The training objective of Jump algorithm (Algorithm~\ref{alg:jump_train}) can be written as:
\begin{align*}
    \mathrm{Loss} = \mathrm{DiffusionLoss} +  \rho  \sum_{i \in [L]}  \sum_{j \in [B]} (p_i(t))_j / B
\end{align*}
where $p_i \in \R^B$ is jumping probability at $i$-th layer and $\rho = 10^{-3}$ is the jump ratio that controls the effect of jumping.
% \Yufa{need to sum over diffusion steps}
Thus, our new loss is the original diffusion loss plus a penalty term that attempts to minimize the times we pass attention/MLP layer.

Overall sparsity for all $T$ steps:
\begin{align*}
    \sum_{t \in [T]} \sum_{i \in [L]}  \sum_{j \in [B]} (p_i(t))_j / B
\end{align*}
We cannot control the overall sparsity. We can only control $\rho$ in the training time.

Diffusion loss = kernel regression

We can prove when adding random jumping (Diffusion loss + penalty term) equivalent to a ridge ($\ell_2$-norm) kernel regression.

\iffalse
\begin{theorem}[Error control, formal version of Theorem~\ref{thm:error:informal}]\label{thm:error:formal}
There exist $\alpha, \epsilon \in (0,0.1)$ such that, if the similarity $f(X_{l,t} , X_{l,t+1}) \geq 1-\alpha$, then $\|X_{l,t} - X_{l,t+1}\|_F \leq \epsilon$. 
\end{theorem}
\fi



Now we can prove the Lipschitz for the two modules. 
We start to prove for single layer DiT which have two consecutive attention and feedfoward layer.
\begin{lemma}[Lipschitz of single layer]\label{lem:lip_single_layer}
If the following conditions hold:
\begin{itemize}
    \item Let $X \in \R^{N \times D}$. 
    \item Let $W^\feed \in \R^{D \times D}$ be defined in Definition~\ref{def:feedforward}.
    \item Let $W, W_V \in \R^{D \times D}$ be defined as in Definition~\ref{def:self_attention}.
    \item $R > 1$ be some fixed constant.
    \item Assume $\|  W^\feed \| \leq R, \|  W \| \leq R, \| W_V \|\leq R, \| X \|\leq R$.
\end{itemize}
Then, we have 
\begin{align*}
    \|\mathcal{F}^\feed_l \circ \mathcal{F}^\attn_l(X) - \mathcal{F}^\feed_l \circ \mathcal{F}^\attn_l(\wt{X})\|\leq 5 R^5 N D \cdot \|X - \wt{X}\|.
\end{align*}
\end{lemma}

\begin{proof}
We can show that
\begin{align*}
    & ~ \|\mathcal{F}^\feed_l \circ \mathcal{F}^\attn_l(X) - \mathcal{F}^\feed_l \circ \mathcal{F}^\attn_l(\wt{X})\|\\
    \leq & ~ R \|\mathcal{F}_l^\attn(X) - \mathcal{F}_l^\attn(\wt{X})\| \\
    \leq & ~ 5 R^5 N D \|X - \wt{X}\|
\end{align*}
where the first step follows from Lemma~\ref{lem:lip_feed}, the second step follows from Lemma~\ref{lem:lip_attn}.
\end{proof}

By mathematical induction and Lemma~\ref{lem:lip_single_layer}, we prove Lipschitz for multi-layer.
\begin{lemma}\label{lem:lipschitz_DiT}
If the following conditions hold:
\begin{itemize}
    \item Let $X \in \R^{N \times D}$. 
    \item Let $W^\feed \in \R^{D \times D}$ be defined in Definition~\ref{def:feedforward}.
    \item Let $W, W_V \in \R^{D \times D}$ be defined as in Definition~\ref{def:self_attention}.
    \item $R > 1$ be some fixed constant.
    \item Assume $\|  W^\feed \| \leq R, \|  W \| \leq R, \| W_V \|\leq R, \| X \|\leq R$.
\end{itemize}
Then, we can show for the whole $L$-layer DiT model $\mathcal{F}$ (Definition~\ref{def:DiT}):
\begin{align*}
    \|\mathcal{F}^{\Phi}(X) - \mathcal{F}^{\Phi}(\wt{X})\| \leq (5 R^5 N D)^L \cdot \|X - \wt{X}\|.
\end{align*}
\end{lemma}

\begin{proof}
We can show that
\begin{align*}
    & ~ \|\mathcal{F}^{\Phi}(X) - \mathcal{F}^{\Phi}(\wt{X})\|  \\
    = & ~ \| \mathcal{F}_L^\feed \circ \mathcal{F}_L^\attn \circ \dots \circ \mathcal{F}_{1}^\feed \circ \mathcal{F}_{1}^\attn (X) - \mathcal{F}_L^\feed \circ \mathcal{F}_L^\attn \circ \dots \circ \mathcal{F}_{1}^\feed \circ \mathcal{F}_{1}^\attn (\wt{X})\|\\
    \leq & ~ 5 R^5 N D \| \mathcal{F}_{L-1}^\feed \circ \mathcal{F}_{L-1}^\attn \circ \dots \circ \mathcal{F}_{1}^\feed \circ \mathcal{F}_{1}^\attn (X) - \mathcal{F}_{L-1}^\feed \circ \mathcal{F}_{L-1}^\attn \circ \dots \circ \mathcal{F}_{1}^\feed \circ \mathcal{F}_{1}^\attn (\wt{X})\|\\
    \leq & ~ (5 R^5 N D)^L \|X - \wt{X}\|
\end{align*}
where the first step follows from Definition~\ref{def:DiT}, the second step from Lemma~\ref{lem:lip_single_layer}, and the last step follows from mathematical induction.
\end{proof}

Furthermore, following the same idea we can show that if input change at any layer or timestep, the whole diffusion process error can be bounded. 
\begin{theorem}[Error control, informal version of Theorem~\ref{thm:lipschitz:informal}]\label{thm:lipschitz:formal}
If the following conditions hold:
\begin{itemize}
    \item Let $X \in \R^{N \times D}$. 
    \item Let $W^\feed \in \R^{D \times D}$ be defined in Definition~\ref{def:feedforward}.
    \item Let $W, W_V \in \R^{D \times D}$ be defined as in Definition~\ref{def:self_attention}.
    \item $R > 1$ be some fixed constant.
    \item Assume $\|  W^\feed \| \leq R, \|  W \| \leq R, \| W_V \|\leq R, \| X \|\leq R$.
\end{itemize}

Suppose we have the $\|\F_k^\Phi(X) - \F_k^\Phi(\wt{X})\| \leq \epsilon$ for $k \in [L]$. 
Then, for total time of $T$ diffusion timesteps, we have the error bounded by
\begin{align*}
    T (5 R^5 N D)^{L - k} \epsilon.
\end{align*}
\end{theorem}

\begin{proof}
We can view $\F_k^\Phi(X)$ as the input for a DiT model with $L - k$ layer.

For $\Phi = \attn$, we can have
From Lemma~\ref{lem:lipschitz_DiT}, we know 
\begin{align*}
     & ~ \| \mathcal{F}_L^\feed \circ \mathcal{F}_L^\attn \circ \dots \circ \mathcal{F}_{k}^\feed \circ \mathcal{F}_{k}^\attn (X) - \mathcal{F}_L^\feed \circ \mathcal{F}_L^\attn \circ \dots \circ \mathcal{F}_{k}^\feed \circ \mathcal{F}_{k}^\attn (\wt{X})\|\\
     \leq & ~ (5 R^5 N D)^{L - k} \cdot \|\F_k^\Phi(X) - \F_k^\Phi(\wt{X})\| \\ 
     \leq & ~ (5 R^5 N D)^{L - k} \epsilon
\end{align*}


For $\Phi = \feed$, the error still apply. Since the attention layer is ahead of Feedforward layer, its error is no more than the error when $\Phi = \attn$.


Then, for one diffusion step, the error can be bounded by $ (5 R^5 N D)^{L - k} \epsilon$.
For total $T$ step, the error magnify a constant of $T$, since we need to pass the same model $T$ time.
\end{proof}









\begin{align*}
    (a+b+c)^{2} \leq 3 \cdot (a^2 + b^2 + c^2)
\end{align*}

% Let $a = {\bf 1}_D \cdot \frac{0.5 \epsilon}{N M_1}$, $b = {\bf 1}_D \cdot \frac{0.5 \epsilon}{N M_2}$, and $c=0$.
% \begin{align*}
%     & ~ \|A \circ X_1 + B \circ X_2 + C \|_F\\
%     \leq & ~ \sum_{i=1}^N \| A_i \circ X_{1,i} + B_i \circ X_{2,i} + C_i \|_2\\
%     = & ~ \sum_{i=1}^N \| a \circ X_{1,i} + b \circ X_{2,i} + c \|_2\\
%     \leq & ~ \sum_{i=1}^N \| a \circ X_{1,i} \|_2 + \|b \circ X_{2,i}\|_2 + \|c\|_2\\
%     = & ~ \sum_{i=1}^N \frac{0.5\epsilon \| X_{1,i}\|}{N M_1} + \frac{0.5\epsilon \| X_{2,i}\|}{N M_2} \\
%     \leq & ~ \sum_{i=1}^N \frac{0.5\epsilon}{N} + \frac{0.5\epsilon}{N}\\
%     = & ~\epsilon
% \end{align*}
% where the first step follows from $\| x \|_2 \leq \| x \|_1$ and $x_i = \| A_i \circ X_{1,i} + B_i \circ X_{2,i} + C_i \|_2$, the second step follows from definition of $A,B,C$, the third step follows from the triangle inequality, the fourth step follows from we define the way we pick $a,b,c$, the fifth step follows from the definition of $M_1,M_2$, the last step follows from basic algebra.

% % {\bf Method 1.}

% % Assume $\| \wt{A}_i \|_2 , \| \wt{B}_i \|_2, \| \wt{C}_i \|_2 \leq \epsilon_0$. 
% % Let $\epsilon_0 = \epsilon /(3N)$. 

% % \begin{align*}
% %     \| \wt{A} + \wt{B} + \wt{C} \|_F \leq & ~ \sum_{i=1}^N \| \wt{A}_i + \wt{B}_i + \wt{C}_i \|_2 \\
% %     \leq & ~ \sum_{i=1}^N \| \wt{A}_i \|_2 + \| \wt{B}_i \|_2 + \| \wt{C}_i \|_2 \\
% %     \leq & ~ 3 N \cdot \epsilon_0 \\
% %     \leq & ~ \epsilon
% % \end{align*}
% % where $\| x \|_2 \leq \| x \|_1$ and $x_i = \| \wt{A}_i + \wt{B}_i + \wt{C}_i \|_2$. 

% {\bf Method 2.}
